Optimal DNN Primitive Selection with Partitioned Boolean Quadratic Programming

Deep Neural Networks (DNNs) require very large amounts of computation both for training and for inference when deployed in the field. Many different algorithms have been proposed to implement the most computationally expensive layers of DNNs. Further, each of these algorithms has a large number of variants, which offer different trade-offs of parallelism, data locality, memory footprint, and execution time. In addition, specific algorithms operate much more efficiently on specialized data layouts and formats. We state the problem of optimal primitive selection in the presence of data format transformations, and show that it is NP-hard by demonstrating an embedding in the Partitioned Boolean Quadratic Assignment problem (PBQP). We propose an analytic solution via a PBQP solver, and evaluate our approach experimentally by optimizing several popular DNNs using a library of more than 70 DNN primitives, on an embedded platform and a general purpose platform. We show experimentally that significant gains are possible versus the state of the art vendor libraries by using a principled analytic solution to the problem of layout selection in the presence of data format transformations.

==> ae-20160509.tex <==
\appendix
\section{Artifact Description}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Abstract}

Our artifacts are delivered as a public Git repository, with a bundled
Dockerfile for our build environment.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Description}

\subsubsection{Check-list (artifact meta information)}

{\small
\begin{itemize}
  \item {\bf Run-time environment: Docker, GNU/Linux}
  \item {\bf Hardware: \texttt{x86\_64} or \texttt{aarch64} CPU}
  \item {\bf Output: measurements as .DAT files, graphs as PDF/EPS files}
  \item {\bf Experiment workflow: make target}
  \item {\bf Publicly available?: yes}
\end{itemize}
}

\subsubsection{How Delivered}

Our library has been released as open-source software under the BSD3 license.

The library and benchmark suite are available in public Git repositories on
Bitbucket; the library is available here
\url{https://bitbucket.org/STG-TCD/trinnity}, and the benchmarks are available
here \url{https://bitbucket.org/STG-TCD/trinnity-benchmarks}.

\subsubsection{Hardware Dependencies}

There are no hardware dependencies, but to reproduce our results exactly, you
will need to use the same platforms as were used in the evaluation in the
paper.

\begin{itemize}
\item Intel Core i5-4570 (Haswell) with min. 8GB RAM
\item NVIDIA Jetson TX1 (ARM Cortex A-57) running \textbf{JetPack 3.0}
\end{itemize}

\subsubsection{Software Dependencies - Docker}
\label{sec:docker}

Our build environment is packaged using Docker. Please make sure
\texttt{docker} is installed, and the docker service is started.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Installation}
\label{sec:install}

Clone the benchmarks using \texttt{git} from the bitbucket repository at
\url{https://bitbucket.org/STG-TCD/cgo-2018-ae}.

Change to the \texttt{trinnity-benchmarks} directory and say \texttt{docker
build -t trinnity-benchmarks -f Dockerfile .} It will take some time to
construct the build environment, but no user interaction is necessary.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experimental Workflow}
\label{sec:bench}

Say \texttt{docker run -i -t trinnity-benchmarks /bin/bash} to start a shell in
our build environment.

If you are running the benchmarking on an \texttt{x86\_64} machine, you will
need to disable ``Intel SpeedStep'' aka Dynamic Voltage and Frequency Scaling,
and ``Intel Turbo Boost'' in BIOS for reproducible benchmark results.
\footnote{\textbf{Please note that simply changing which run-time CPU governor
is enabled will not suffice}. In addition, you may need to disable the
\texttt{intel\_pstate} kernel module, by editing your boot loader configuration
and placing the command \texttt{intel\_pstate=disable} at the end of the kernel
boot line (which should start with \texttt{linux}). This will require a
reboot.}

NVIDIA provide a setup script for the Jetson TX1 called
\texttt{jetson-clocks.sh} in the home directory which places the device in
high-performance mode. This script should be executed as \texttt{root} before
running the benchmarks on the TX1.

Graphs are produced in the \texttt{build/graphs} subdirectory.

\subsubsection{CGO AE Benchmarking}

We have provided special \texttt{make} targets which step through the
benchmarking used to generate the graphs in our paper, all the way from initial
microbenchmarking to construct the cost models, to building the final optimized
network executables, timing, and plotting the results.

To begin the benchmarking process, create an empty \texttt{Makefile.config}
by executing the command

\texttt{touch Makefile.config}.

\noindent To run the end-to-end benchmarking process, say

\texttt{make end-to-end-cgo-x86\_64}

\noindent if you are on an \texttt{x86\_64} machine.

\subsubsection{Cross Compilation}

While you can run the end-to-end benchmarking process on the TX1 system, it is
much faster to build the benchmarks by cross-compilation on a more powerful
system.

On your \texttt{x86\_64} machine, build the cost model microbenchmarks by
executing

\texttt{make\\
end-to-end-cgo-aarch64-build-cost-model-progs}

\noindent then copy the whole \texttt{triNNity-benchmarks} directory to the
\texttt{aarch64} test machine (for example, with

\texttt{rsync -avP ./ user@aarch64-machine:dir})

\noindent and on your \texttt{aarch64} machine, execute

\texttt{make end-to-end-cgo-aarch64-build-cost-model}

\noindent to build the cost model. Copy the directory back to your
\texttt{x86\_64} machine, and say

\texttt{make end-to-end-cgo-aarch64-networks-build}

\noindent to cross-compile the benchmarks using the cost model built on
\texttt{aarch64}. After this, you can copy the directory once more to the
\texttt{aarch64} machine, and say

\texttt{make end-to-end-cgo-aarch64-networks-run}

\noindent to run the benchmarks and produce the final graphs.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evaluation and Expected Results}

The directory \texttt{build/graphs} will contain the graphs produced from
whole-network benchmarking. These should correspond very closely to those in
the paper.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment Customization}

Extensive customization is possible, but should not be necessary. The entire
benchmark build system is contained in the Makefile, which builds the workflow
up in simple steps which invoke other make rules in
sequence.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% When adding this appendix to your paper,
% please remove below part
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

